Stability and Scalability of Blockchain Systems

The blockchain paradigm provides a mechanism for content dissemination and distributed consensus on Peer-to-Peer (P2P) networks. While this paradigm has been widely adopted in industry, it has not been carefully analyzed in terms of its network scaling with respect to the number of peers. Applications for blockchain systems, such as cryptocurrencies and IoT, require this form of network scaling. In this paper, we propose a new stochastic network model for a blockchain system. We identify a structural property called \emph{one-endedness}, which we show to be desirable in any blockchain system as it is directly related to distributed consensus among the peers. We show that the stochastic stability of the network is sufficient for the one-endedness of a blockchain. We further establish that our model belongs to a class of network models, called monotone separable models. This allows us to establish upper and lower bounds on the stability region. The bounds on stability depend on the connectivity of the P2P network through its conductance and allow us to analyze the scalability of blockchain systems on large P2P networks. We verify our theoretical insights using both synthetic data and real data from the Bitcoin network.

==> figs/torus-figure.tex <==
{\centering
  \begin{tikzpicture}[scale=0.5]
  
  \draw [-, thick] (-1, 0) -- (1, 0);
  \draw [-, thick] (-1, 0) -- (2, -1.732);
  \draw [-, thick] (1, 0) -- (2, -1.732);
  \draw [-, thick] (1, 0) -- (1, -3.464);
  \draw [-, thick] (2, -1.732) -- (1, -3.464);
  \draw [-, thick] (2, -1.732) -- (-1, -3.464);
  \draw [-, thick] (1, -3.464) -- (-1, -3.464);
  \draw [-, thick] (1, -3.464) -- (-2, -1.732);
  \draw [-, thick] (-1, -3.464) -- (-2, -1.732);
  \draw [-, thick] (-1, -3.464) -- (-1, 0);
  \draw [-, thick] (-2, -1.732) -- (-1, 0);
  \draw [-, thick] (-2, -1.732) -- (1, 0);
  
  \draw[fill=white] (-1, 0) circle [radius=0.375];
  \node at (-1, 0) {$1$};
  \draw[fill=white] (1, 0) circle [radius=0.375];
  \node at (1, 0) {$2$};
  \draw[fill=white] (2, -1.732) circle [radius=0.375];
  \node at (2, -1.732) {$3$};
  \draw[fill=white] (1, -3.464) circle [radius=0.375];
  \node at (1, -3.464) {$4$};
  \draw[fill=white] (-1, -3.464) circle [radius=0.375];
  \node at (-1, -3.464) {$5$};
  \draw[fill=white] (-2, -1.732) circle [radius=0.375];
  \node at (-2, -1.732) {$6$};
  \end{tikzpicture}  
}

==> main.tex <==
%\input{main-submission.tex}
\input{main-pre-publication.tex}
%\input{main-extended-abstract}

==> scalability.tex <==
\section{Scalability of Common Network Topologies}
\label{sec:scalability}
In this section, we examine the scalability of blockchain systems under common network topologies -- namely, we study the blockchain dynamics on a sequence of peer-to-peer networks with increasing numbers of peers. 
% The goal is to analyze blockchain dynamics in the limit as the number of peers tends to infinity.
%We do so by considering the peer-to-peer network $H$ to belong to various families of network topologies and their conductances as $N\to\infty$, thus determining the potential scalability for blockchain systems.}
Recall that a blockchain system is \emph{scalable} on a sequence of networks $(H_k)_{k\in\mathbb{N}}$, where the number of peers in $H_k$ grows monotonically with $k$, if there exists a positive block arrival rate $\lambda^* > 0$ such that for all $k\in\mathbb{N}$, the blockchain system on network $H_k$ is stable for $\lambda^*$.
Theorem \ref{thm:stability} shows that for any peer-to-peer network $H$, the maximal block arrival rate into the network is bounded below and above by $\frac{\phi_H}{2\log(N)}$ and $\phi_H$, respectively. 

\begin{remark}
  For any connected peer-to-peer network $H$, the conductance $\phi_H$ is bounded above by 2.
  This can be seen by taking the set $S$ in Definition \ref{def:conductance} such that it contains exactly one vertex.
  As a result, it follows that the per-peer block arrival rate must decrease to zero as $N\to\infty$ if stability is to be maintained.
  
  Nevertheless, the blockchain system is scalable if there exists a positive \textit{global} block arrival rate $\lambda^*$ such that all peer-to-peer networks $(H_k)_{k \in \mathbb{N}}$ are stable.
  Thus, from the bounds in Theorem \ref{thm:stability}, a necessary condition for a family of networks $(H_k)_k$ to be scalable is that $\lim_{k \to \infty}\phi_{H_k} > 0$.
\end{remark}

In the rest of the section, we consider various network families and analyze their limiting conductances to assess scalability.

\subsection{Regular Grids}
In this subsection we consider regular grids on tori.
% Such graph models are typically used to study network processes with geographic locality, such as wireless networks {\color{red} CITE HERE franceschetti and david tse}.
Concretely, given $k \in \mathbb{N}$ and a dimension $d \in \mathbb{N}$, we consider the $d$-dimensional torus with $N$ vertices and edges between any two vertices $v_1, v_2$ if the grid distance $D(v_1, v_2) \leq k$, denoted by $H_N^{(d)}$: $H_N^{(d)} = [0, \lfloor N^{\frac{1}{d}} \rfloor]^d.$

An example of the torus $H_6^{(1)}$ with $k = 2$ dimensions is given below in Figure \ref{fig:torus}. 
\begin{figure}
    \centering
    \input{figs/torus-figure.tex}
    \caption{The torus $H_6^{(1)}$ with $k = 2$.}
    \label{fig:torus}
\end{figure}

It is well known that for any fixed dimension $d$ and constant $k$, as $N\to\infty$, the conductances of the torus $H_N^{(k)}$ and also the grid, decrease to $0$ \cite{lyons2017probability}.

% In this section, we consider grid like graphs. Concretely, given a $k \in \mathbb{N}$ and $d \in \mathbb{N}$, we first consider the torus $H_N^{(1)}$ on $\mathbb{Z}^d$, i.e., $[0,\lfloor N^{1/d} \rfloor]^d$. 
% For instance if $d=2$, then the torus corresponds to the subgraph of the two dimensional grid restricted to $[0,\lfloor \sqrt{n} \rfloor] \times [0,\lfloor \sqrt{n} \rfloor]$.
% Thus, the graph $H_N^{(1)}$ is the grid (torus) in $d$ dimensions with $N$ vertices. We further identify the ends and consider the torus $H_N^{(1)}$. For any $k \in \mathbb{N}$, we add an edge between vertices $i,j \in H_N^{(k)}$, if the graph distance between $i$ and $j$ in the torus $H_N^{(1)}$ is less than or equal to $k$. 
% We consider such graphs as they are usually used as models to study networks with geographic locality, typical in wireless networks \cite{grid-networks}.
% Standard results gives that \cite{conductance-geometric}, that for any fixed $k,d$, the conductance $\phi_{H_N^{(k)}}\to0$ as $N\to \infty$. Notice, that this is a family of determinisitic graphs.

\subsection{Regular Trees}
Consider the $d$-regular tree with depth $k$.
Recall that the $d$-regular tree has a single vertex of degree $d-1$ called the \emph{root}; each vertex that is not a leaf has $d-1$ children. 
Thus, the total number of vertices in the $d$-regular tree of depth $k$ is $\sum_{i = 0}^{k}{d^i} = \frac{d^{k+1}-1}{d-1}$.

Let $H_k$ be the $d$-regular tree with $k$ layers and consider the following cut.
As per Definition \ref{def:conductance}, let the set $S$ contain the root and all the descendants of all but one of the root's children. 
Thus the root in the set $S$ has degree $d-2$.
The conductance of this cut is $\frac{\frac{1}{d-1}}{\frac1N(1 + \frac{d-2}{d-1}(N-1))(\frac{1}{d-1}(N-1))}$, which tends to $0$ as the depth $k\to\infty$.
Thus the sequence $(H_k)_k$ of $d$-regular trees of depth $k$ is not scalable.

\subsection{Erd\"os-R\'enyi Networks}
In this subsection we consider the simplest model of random networks, the Erd\"os-R\'enyi model.
In this model, the network $H_N$ consists of $N$ vertices, and each pair of vertices $v_1, v_2$ are connected by an edge independently with some probability $p$.
It is well known that if $p > \frac{C\log N}{N}$, for any fixed $C > 1$, that the Erd\"os-R\'enyi network on $N$ vertices is connected with high probability \cite{janson2011random}.
The network sequence $(H_N)_{N \geq 1}$ is a sequence of random networks, with $H_N$ being distributed as the largest connected component in $G(N,p)$, where $p > \frac{C\log N}{N}$, with $C > 1$.
For this model, there exists $\varepsilon > 0$, which depends on $C$, such that $\lim_{N\to\infty}\mathbb{P}[\phi_{H_N} \geq \varepsilon] = 1$ \cite{janson2011random}.
In particular this implies that the limiting conductance of the sequence of networks $(H_N)_N$ is greater than $0$; in this case we cannot conclusively determine the scalability of blockchain systems using Theorem \ref{thm:stability}.

% Consider the simplest model of random graphs, where $(H_N)_{N \geq 1}$ is a sequence of random graphs, where for each $N \geq 1$, each of the ${N \choose 2}$ potential edges of $H_N$ are chosen independently with probability $\frac{C \log(N)}{N}$, for some fixed parameter $C > 1$. Standard results \cite{janson2011random} give that $\lim_{N \rightarrow \infty} \mathbb{P}[H_N \text{ is connected}]=1$. For this model again, \cite{er-conductance} gives that there exists a $\varepsilon > 0$, depending on $C$, such that $\mathbb{P}[\phi_{H_N} \geq \varepsilon] = 1$, i.e., the conductance is bounded away from $0$. Thus, again we cannot exactly determine the scalability properties in this case.

\subsection{Random $d$-regular Networks}

Suppose that for each $N \geq 1$, $H_N$ is a random $d$-regular network for some fixed $d \geq 3$ (\cite{janson2011random}). 
Krivelevich \textit{et al.} show that for every $\varepsilon > 0$ and $d \geq 3$, $\lim_{N \rightarrow \infty}\mathbb{P}[\phi_{H_N} \geq 1-\varepsilon] = 1$ \cite{krivelevich2001random}. 
In particular, it cannot be conclusively determined from Theorem \ref{thm:stability} whether or not sequences of $d$-regular random networks are scalable.

\subsection{Preferential Attachment Networks}

We next consider a class of random networks with power law degree distributions called preferential attachment networks \cite{van2009random}.
It is widely reported that the network structure of the World Wide Web can be modeled by preferential attachment type models \cite{newman2018networks, faloustos1999power}.
% A common random graph model to study power law degree distributions is the preferential attachment model \cite{van2009random}.
We consider the preferential attachment model described in \cite{mihail2003certain}.
Roughly speaking, the network $H_N$ is constructed as follows. 
Initially there is a single vertex with a self loop.
For some $d \geq 2$, a parameter of the model, $dN$ vertices are added sequentially.
Each arriving vertex picks one of the existing vertices with probability proportional to the degree at the time of arrival.
This produces a tree (denoted by $T_{dN}$), after all $dN$ vertices are added.
The network $H_N$ is then obtained by shrinking the vertices of $T_{dN}$, namely, for all $1 \leq i \leq N$, all vertices indexed $di \leq j < (d+1)i$ of $T_{dN}$ are considered as a single vertex of $G_n$, with the associated edges and self loops and multiple edges retained from this construction.

% {\color{orange}Note that this construction differs from the more standard definition of preferential attachment given in \cite{van2009random, chierichetti2010rumour} due to the presence of self-loops and multiple edges; however, the conductance of the construction in \cite{van2009random, chierichetti2010rumour} is an open question.}

It is shown in \cite{mihail2003certain} that there exists a $\varepsilon > 0$, such that \\ $\lim_{N\to\infty}\mathbb{P}[\phi_{H_N} > \varepsilon] = 1.$
Thus, we cannot conclusively assess scalability for this class of networks.

% The conductance of this family of graphs defined in \cite{mihail2003certain} is shown to be bounded away from $0$, namely, with probability going to $1$ as $N$ goes to infinity, there exists a $\varepsilon > 0$, such that $\lim_{N \rightarrow \infty}\mathbb{P}[\phi_{H_N} \geq \varepsilon]$. 
% Thus, for this family of graphs, we cannot conclusively assess scalability.

\subsection{Random Geometric Networks}

A random geometric network on $N$ vertices is constructed by independently and uniformly selecting $N$ points in the plane $[0, 1]\times[0, 1]$, and adding an edge between any two vertices whose Euclidean distance is less than some positive fixed radius $r > 0$ \cite{penrose2003random}.
Penrose \textit{et al.} \cite{penrose2003random} show that for any positive constant $C > 1$, the random geometric networks $(H_N)_N$ with radii $r_N = C\sqrt{\frac{\log N}{N}}$ are connected with high probability.

Random geometric networks are well-suited to model networks with geographic locality, such as peer-to-peer networks \cite{baccelli2013p2p} and wireless networks \cite{tse2005fundamentals}.
Due to the spatial embedding of this class of networks, it is known that for any fixed $C > 1$, the conductance of the largest connected component of $\phi_{H_N}$, tends to $0$; \textit{i.e.}, $\lim_{N\to\infty}\mathbb{P}[\phi_{H_N} \geq \varepsilon] = 0$, for all $\varepsilon  > 0$ \cite{penrose2003random}.
As a result, this class of connected random geometric networks is non-scalable.


% This class of graphs are a randomized version of the aforementiond grids. Concretely, the graph $H_N$ is constructed by first assigning to each of the $N$ vertices, a spatial label chosen uniformly and independently at random from the $2$ dimensionsl unit box $[0,1]\times[0,1]$. Subsequently, an edge is placed between two vertices if and only if their distance is smaller than or equal to a threshold $C \sqrt{\frac{\log(N)}{N}}$, for some $C>0$, which is a fixed parameter. Standard results (\cite{penrose2003random}, gives that if $C > 1$, then with high probability, the random graph is connected. However, due to the spatial embedding of this graphs, it is easy to show that (see \cite{penrose2003random}), for any fixed $C > 0$, the conductances $\phi_{H_N}\to 0$, almost surely as $N\to \infty$. Thus, again, this class of graphs, are not scalable. This is of particular importance, as geometric graphs models are shown to model real world peer-to-peer networks well \cite{baccelli2013p2p}. This follows as peers are likely to connect with other peers with whom they have low network latency, thus using ``ping'' as a distance metric.


% ---------

% OLD CONTENT Introductory text
% Section 4 identifies the \emph{maximum block rate} as a key metric for analyzing blockchain scalability as an intrinsic property of any peer to peer network $H$.
% In this section, we provide lower and upper bounds on the maximum block rate.


% \begin{remark}[Maximum Block Rate vs. Transactions per Second]
%     Traditional blockchain literature {\color{red}TODO: cites} use the metric of \emph{transactions per second (TPS)} as a measure of network performance and scalability in blockchain and blockchain-like systems.
%     However, as a result of Theorem \ref{thm:stability}, the metric of Transactions per Second is a function of both the maximum block rate and the edge selection rule -- for example, choosing either of the last two examples of edge selection rules results in more block throughput than using the first (where block throughput in the limit is the fraction of vertices that have infinitely many vertices pointing to them).

%     As such we use the term \emph{scalability} to study whether or not there exist positive block rates $r$ such that in the limit as $N\rightarrow\infty$, a block rate of $r$ remains stable in terms of the communication process; if not it is important to understand the rate at which the maximum block rate decreases with network size.
% \end{remark}

% \subsection{Bounds on the Stability Region of Longest-Chain Blockchains}
% {\color{red} TODO: don't need this until the theorem}
% In this subsection we assume that the processes $E, T_{p}, p \in \{1, 2, \ldots, N\}$ are stationary and ergodic, and mutually independent. 
% Thus the quantities $\mathbb{E}[C_k - C_{k-1}]$ are equal for all $k$ and we use the notation $\bar{C}$ to refer to $\mathbb{E}[C_2 - C_1]$ as the time to consistency.


% Further, we assume that for each peer $p$ the marks of the point process $T_p$ are independently and uniformly selected among the neighbors of $p$ and $E$ is such that the arrival rates each peer are uniform.
% This is similar to other gossip-based models in Peer-to-Peer literature such as {\color{red} TODO: cites (sanghavi, shah, etc.)}

% Under these additional assumptions, we proceed to examine the dynamics on the P2P system under the framework of \emph{monotone separability} \cite{baccelli1995saturation}.
% This framework allows us to determine lower and upper bounds on the critical arrival rate $\lambda_C^H$ for the process $E$ below which the communication process on $H$ is stable and thus the limiting graph is one-ended by Theorem \ref{thm:stability}.

% We denote by $E_m$ the $m$-th arrival of $E$, which is vertex $m$ of $G(t)$. 
% If the arrival $E_m$ arrives to an empty system, let $X_{[m, n]}(E)$ denote the earliest time when $B_p(t) = \{m, \ldots, n\} \ \forall p$.
% In other words, $X_{[m, n]}(E)$ denotes the first time of consistency such that all peers are consistent on the blocks $\{m, \ldots, n\}$.


% A system is monotone separable if it satisfies the following four requirements when $m \leq n$ and $m \leq l < n$:
% \begin{enumerate}
%     \item (causality) $X_{[m, n]}(E) \geq E_n$
%     \item (external monotonicity) $X_{[m, n]}(E') \geq X_{[m, n]}(E)$ whenever $E'$ is a point process such that $E' \geq E$
%     \item (homogeneity) $X_{[m, n]}(E + c) = X_{[m, n]}(E) + c \ \forall c \in \mathbb{R}$
%     \item (separability) $X_{[m, n]}(E) = X_{[l+1, n]}(E)$ if $X_{[m, l]}(E) \leq E_{l+1}$.
% \end{enumerate}

% Baccelli and Foss prove that monotone separable systems are stable (that is, the time to consistency is finite a.s.) when the arrival rate is less than $\gamma_0^{-1}$, where $\gamma_0 = \lim_{n\rightarrow\infty} \frac{X_n}{n}$, and $X_n$ is the time to consistency when $n$ blocks arrive to the system at time 0 ($X_n$ is also known as the maximal dater in the queueing theory literature) \cite{baccelli1995saturation}.
% In essence, the monotone separability framework allows us to shift arrivals in time to deduce bounds on the critical arrival rate to the system.

% \begin{lemma}
%     With the added requirements of this section, the communication dynamics are monotone separable.
%     \label{lem:monotone_separability}
% \end{lemma}
% \begin{proof}
%     We denote by $E_n$ the $n-th$ exogenous block arrival for the arrival process $E$.
%     $E$ is a marked point process, such that the mark of $E_n$ consists of two parts:
%     \begin{enumerate}
%         \item the peer to which it arrives
%         \item the the evolution of $T$, restricted to transmission clicks which occur after $E_n$
%     \end{enumerate}
    
    
%     We show that blockchain-like systems, under the assumptions added in this section, exhibit these properties now.
%     \begin{enumerate}
%         \item (causality) As each block arrives to exactly one peer and the processes $T_i$ are all of finite non-zero rate, it follows that at least $n-1$ clicks are necessary after $E_n$ in order to reach a time to consistency; thus the system is causal as $X_{[m, n]}(E) > E_n$ a.s..
%         \item (external monotonocity) This follows from the FCFS nature of the gossiping process.
%         Namely, for each block, delaying its arrival may increase the number of vertices to be informed of the block while the block is the oldest in the system, thus increasing its exit time.
        
%         Actual proof:
%         {\color{red} TODO come back and fill in}
%         \item (homogeneity) As the gossiping processes are FCFS, let $\tau$ be the time from the arrival of $E_n$ until consistency.
%         Note that $\tau$ is time-invariant as it is derived from the mark of $E_n$.
%         Then $X_{[m, n]}(E) + c = (E_n + \tau) + c = (E_n + c) + \tau = X_{[m, n]}(E + c)$.
%         \item (separability) By assumption block $E_{l+1}$ arrives at an empty system; thus block $E_n$ does not wait for the dispersal of any of the blocks $E_m, E_{m+1}, \ldots E_l$ due to the FCFS nature of the gossiping process.
%         It follows that $X_{[m, n]}(E) = X_{[l+1, n]}(E)$.
%     \end{enumerate}
% \end{proof}

% Before we bound the intensity of $E$ we first define the \emph{conductance} of the Peer-to-Peer network $H$, which measures the susceptibility of the communication process to peers who may act as bottlenecks due to the structure of $H$ -- networks with lower conductance are more susceptible to bottlenecks.
% \begin{definition}
%     Let $(S, S^C)$ be a cut of $H$.
%     The conductance of the cut $\phi_{(S, S^C)}$ is given by 
%     $$
%         \phi_{(S, S^C)} = \frac{\sum_{p \in S, q \in S^C, (p, q) \in H}\frac{1}{d(p)}}{\frac{1}{N}|S||S^C|},
%     $$
%     where $d(p)$ is the degree of peer $p$ and $|\cdot|$ is the cardinality of $\cdot$.
    
%     The conductance $\phi_H$ of $H$ is given by the infimum of the conductance of any cut.
% \end{definition}
% Note that the conductance of any network $H$ with $N$ vertices is at most the conductance of $K_N$ which is 1.

% We now proceed to bound the arrival rate of $E$ such that the communication dynamics are stable.

% \begin{theorem}
%   Let $\phi_H$ be the conductance of the Peer-to-Peer network $H$.
%   If the point processes $T_p$ are mutually independent for all $p \in \{1, 2, \ldots, N\}$, the critical arrival rate $\lambda_C^H$ such that $\bar{C}$ is finite a.s. satisfies $O(\frac{\phi_H}{\log N}) \leq \lambda_C^H \leq O(\phi_H)$.
%   In particular, no blockchain is scalable under the assumptions of this paper.
%   \label{thm:scalability}
% \end{theorem}
% \begin{proof}
%     The system is monotone separable from Lemma \ref{lem:monotone_separability}.
%     As such, we proceed by providing lower bounds and upper bounds for $X_n$ and taking the limit $n\rightarrow\infty$.
    
%     Ganesh \cite{ganeshnotes} gives an upper bound for $\mathbb{E}[X_1] \leq \frac{2\log N}{\phi_H}$.
%     By monotone separability, we shift the arrivals so that each arrival occurs at the exact instant the previous arrival is known to all peers.
%     Thus, by the strong law of large numbers, we have:
%     \begin{equation}
%         \gamma_0 = \lim_{n\rightarrow\infty}\frac{X_n}{n} = \frac{2\log N}{\phi_H}
%     \end{equation}
%     and so a lower bound on the critical arrival rate is
%     \begin{equation}
%         O(\frac{\phi_H}{\log N}) \leq \lambda_C^H.
%     \end{equation}
    
%     If $(S, S^C)$ is a cut of $H$ and $S$ is non-empty, we note that the clearing time $X_n$ for $n$ packets is at least as long as the time it takes for all the vertices initially at vertices in $S$ to be communicated to vertices in $S^C$.
%     By definition, the cut used in computing the conductance of $H$ is minimal in the sense that it is the cut which minimizes the rate of communication between the resulting two subgraphs of $H$; thus this cut allows us to compute the supremum over cuts of the clearing time $X_n$.
%     Let $(S, S^C)$ be a cut with minimal conductance where $|S| \geq |S^C|$.
%     Shifting the arrivals so that they all occur at time 0, we have:
%     \begin{equation}
%         X_n \geq \frac{n|S|}{N}\frac{1}{\sum_{p \in S, q \in S^C}\frac{1}{d(p)}}
%         = \frac{n}{|S^C|}\frac{1}{\phi_H};
%     \end{equation}
%     thus 
%     \begin{equation}
%         \gamma_0 = \lim_{n\rightarrow\infty} \frac{X_n}{n} \geq \frac{1}{|S^C|\phi_H}.
%     \end{equation}
%     Thus, it follows that an upper bound on the critical vertex arrival rate is $\lambda_C^N \leq |S^C|\phi_H$. Since, this is true for all non-empty sets $S$, we can make the bound tight by choosing $|S^{C}|=1$, which yields that $\lambda_C^{H} \leq \phi_H$.
% \end{proof}

% Theorem \ref{thm:scalability} establishes that blockchains built with communication protocols based on the traditional gossip model for peer-to-peer networks are not scalable; namely for any positive block arrival rate $\lambda$ there is a constant $N_\lambda$ above which the communication protocol ceases to be positive recurrent.

==> shepherd-rebuttal.tex <==
\section{Response to the Shepherd}
In this section we address the shepherd comments prior to publication.
Again, we thank the reviewers for their comments on both the first and revised submissions for this paper.

\subsection{Clarifying the Notion of Limiting Graph}
In the (revised) submission, we defined the DAG $G(\infty) := \bigcup_{t \geq 0} \bigcup_{p \in [N]}G_p(t)$.
Observe that, almost-surely, in any interval of $[0,t]$, there are only finitely many events (block arrivals) occur. Thus, with probability $1$, the definition $G(\infty)$ is a countable union and hence is almost surely well defined.
Nevertheless, we call $G(\infty)$ a \emph{limiting blockchain DAG} as it is shown in Appendix \ref{app:technical-dag} that $G(\infty)$ is an appropriate limit of finite DAGs.
Note that $G(\infty)$ is the only infinite DAG considered in this paper. 
All other DAGs, such as $G(t)$ and $G_p(t)$ are finite for any $t < \infty$.

\subsection{The Role of the P2P Network}
Reviewer C pointed out that for the experiment we did, the numerical results are similar for all of the network topologies we considered.
This is due to the fact that in Bitcoin, the block arrival rate is on average 1 block per 600 seconds, while propagating a typical block takes ~40 seconds $\cite{decker2013information}$ for the current network size.
However, our simulation results suggest that the network topology plays a key role in blockchain performance, when the block propagation delay is larger.
This is expected to occur with massive adoption of blockchain technologies, that increase network sizes and thus also increase block propagation delay.

\subsection{Other Comments}
We have edited the paper to reflect the following points.
\begin{enumerate}
    \item Added to the introduction the fact that the key identifying feature of a blockchain system is that the causal relationship between blocks enforces that all peers should be made aware of all blocks.
    As this is the key feature, we only study blockchains insofar as this feature affects performance.
    \item Added a new reference to the related work section.
    \item Added in the relevant discussions from the previous rebuttal to the body of the paper.
\end{enumerate}

\subsection{Title of the Paper}
We believe the current title of this paper, ``Stability and Scalability of Blockchain Systems,'' to be the best choice of title.
In particular, we note that our paper studies the key aspects which enable a blockchain system to confirm blocks, a discussion of which we added to the Introduction.
While peer-to-peer networks are a key component in blockchain systems, the dynamics on the network are different from what has been studied and from what is typically implied by a process on a peer-to-peer network.
The additional causal relationship between blocks and the eventual one-endedness property is unrelated to peer-to-peer networks.

Further, there are many open questions resulting from our work, all of which directly relate to a better understanding of the stability and scalability of blockchain systems.
We feel the present title highlights both the importance of our results for the general blockchain space as well as the importance of this future work for blockchain system design.
We feel that amending the title of this paper to include the term ``peer-to-peer'' or any equivalent is a dis-service to our contributions (taken in total) as well as to the significance of this future work.

